Robust Covariance Matrix Estimation for Radar Space-Time Adaptive Processing (STAP)

Estimating the disturbance or clutter covariance is a centrally important problem in radar space time adaptive processing (STAP). The disturbance covariance matrix should be inferred from training sample observations in practice. Large number of homogeneous training samples are generally not available because of difficulty of guaranteeing target free disturbance observation, practical limitations imposed by the spatio-temporal nonstationarity, and system considerations. In this dissertation, we look to address the aforementioned challenges by exploiting physically inspired constraints into ML estimation. While adding constraints is beneficial to achieve satisfactory performance in the practical regime of limited training, it leads to a challenging problem. We focus on breaking this classical trade-off between computational tractability and desirable performance measures, particularly in training starved regimes. In particular, we exploit both the structure of the disturbance covariance and importantly the knowledge of the clutter rank to yield a new rank constrained maximum likelihood (RCML) estimator. In addition, we derive a new covariance estimator for STAP that jointly considers a Toeplitz structure and a rank constraint on the clutter component. Finally, we address the problem of working with inexact physical radar parameters under a practical radar environment. We propose a robust covariance estimation method via an expected likelihood (EL) approach. We analyze covariance estimation algorithms under three different cases of imperfect constraints: 1) only rank constraint, 2) both rank and noise power constraint, and 3) condition number constraint. For each case, we formulate estimation of the constraint as an optimization problem with the EL criterion and formally derive and prove a significant analytical result such as uniqueness of the solution.

==> eqparbox/README <==
                  +--------------------------------+
                  |EQPARBOX: Equal-widthed parboxes|
                  |By Scott Pakin <pakin@uiuc.edu> |
                  +--------------------------------+


Description
-----------

LaTeX users sometimes need to ensure that two or more blocks of text
occupy the same amount of horizontal space on the page.  To that end,
the eqparbox package defines a new command, \eqparbox, which works
just like \parbox, except that instead of specifying a width, one
specifies a tag.  All eqparboxes with the same tag -- regardless of
where they are in the document -- will stretch to fit the widest
eqparbox with that tag.  This simple, equal-width mechanism can be
used for a variety of alignment purposes, as is evidenced by the
examples in eqparbox's documentation.


Installation
------------

There's nothing special about building eqparbox:

    latex eqparbox.ins     <== Generate eqparbox.sty
    latex eqparbox.dtx     <== Produce the documentation (eqparbox.dvi)
    latex eqparbox.dtx     <== Again, to get labels and eqparboxes right
    makeindex -s gind.ist eqparbox    <== Generate an index
    latex eqparbox.dtx     <== Incorporate the index into the document

If you're new to this, see
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=instpackages for more
information on installing packages.


Copyright and license
---------------------
Copyright (C) 2001 Scott Pakin <pakin@uiuc.edu>

This package may be distributed and/or modified under the conditions
of the LaTeX Project Public License, either version 1.2 of this
license or (at your option) any later version.  The latest version of
this license is in:

    http://www.latex-project.org/lppl.txt

and version 1.2 or later is part of all distributions of LaTeX version
1999/12/01 or later.

